Efficient First-Order Algorithms for Adaptive Signal Denoising

We consider the problem of discrete-time signal denoising, focusing on a specific family of non-linear convolution-type estimators. Each such estimator is associated with a time-invariant filter which is obtained adaptively, by solving a certain convex optimization problem. Adaptive convolution-type estimators were demonstrated to have favorable statistical properties. However, the question of their computational complexity remains largely unexplored, and in fact we are not aware of any publicly available implementation of these estimators. Our first contribution is an efficient implementation of these estimators via some known first-order proximal algorithms. Our second contribution is a computational complexity analysis of the proposed procedures, which takes into account their statistical nature and the related notion of statistical accuracy. The proposed procedures and their analysis are illustrated on a simulated data benchmark.

==> extra-exp-real.tex <==
\paragraph{Real-data experiments using Lepski's method.}
Here we evaluate our approach on some real-world music sounds and speech samples. Namely, we denoise the following as suggested in~\cite{yu2008audio}.
\begin{itemize}
\item[-] a piano key stroke (C key of the 1st octave); 
\item[-] male and female utterances in Cantonese from the TIMIT database;
\item[-] a short excerpt from Mozart's Oboe Concerto in C major. 
\end{itemize}

==> intro_conflict.tex <==
\section{Introduction and Related Work} %\dimacorr{}{3$\to$2.25?}
\label{sec:intro}

In this paper, we consider the problem of discrete-time signal denosing.
%It can be stated as follows.
%Let $\C(\Z)$ denote the space of all two-sided sequences of complex numbers, and 
The goal is to estimate an unknown complex discrete-time signal $x = (x_\tau)$, $\tau \in \Z$, from observations $y = (y_\tau)$ in complex Gaussian noise:
\begin{equation}
\label{eq:intro-observations}
y_\tau := x_\tau + \sigma \zeta_\tau, \quad \tau = -n, ..., n.
\end{equation}
Here, $\zeta_\tau$ are i.i.d. random variables with standard complex Gaussian distribution $\C\N(0,1)$, meaning that the real and imaginary parts of $\zeta_\tau$ are independent standard Gaussian random variables.
Before proceeding further, let us introduce the necessary notation.

\paragraph{Notation.}
We denote $\C(\Z)$ the space of all complex-valued signals on $\Z$, or, simply, the space of all two-sided complex sequences.
We call $\C_n(\Z)$ the finite-dimensional subspace of $\C(\Z)$ consisting of signals supported on $[0, n]$:
\[
\C_n(\Z) = \left\{(x_\tau) \in \C(\Z): x_\tau = 0 \; \text{ whenever} \;  \tau \notin [0,n] \right\};
\]
its counterpart $\C_n^{\pm}(\Z)$ consists of all signals supported on $[-n, n]$. 
The unknown signal will be assumed to come from one of such subspaces, which corresponds to a finite signal length.
%In particular, $\C_\infty$ is simply the space of all two-sided infinite complex sequencies.
Note that the signals from $\C(\Z)$ can be naturally mapped to column vectors by means of the index-restriction operator $[\cdot]_{m}^n$ defined for any $m, n \in \Z$ such that $m \le n$:
\[
[x]_{m}^n \in \C^{n-m+1}.
\]
In particular, $[\cdot]_{0}^n$ and $[\cdot]_{-n}^n$ define, correspondingly, one-to-one mappings $\C_n(\Z) \to \C^{n+1}$ and $\C_n^\pm(\Z) \to \C^{2n+1}$.
For convenience, column-vectors in $\C^{n+1}$ and $\C^{2n+1}$ will be indexed starting from zero. 
%As such, it will be convenient for us to index vectors in $\C^{N+1}$ (and $\R^{N+1}$) starting from zero, and identify $\C_n^+$ with $\C^{n+1}$.
We define the scaled $\ell_p$-seminorms on $\C(\Z)$:
\[
\| x \|_{n,p} := \frac{\|[x]_{0}^n\|_p}{(n+1)^{1/p}} = \left(\frac{1}{n+1}\sum_{\tau = 0}^n |x_\tau|^{p} \right)^{\frac{1}{p}}, \;  p \ge 1.
\]
%Note that notation $\C^N$ -- with a superscript -- is standard; it is used to distinguish column-vectors, which are always indexed starting with $1$, from ``signals'' which can be indexed on any subset of $\Z$. 
%In particular, in the matrix-vector multiplication we always use column-vectors in $\C^N$ for some $N \in \mathbb{N}$, rather than signals in $\C_n^{\vphantom{+}}$ or $\C_n^+$.
%The goal is to estimate the signal, that is, to construct some $\widehat x \in \C(\Z)$ from the observations~\eqref{eq:intro-observations} that is close to $x$ in some sense. 
We use the ``Matlab notation'' for matrix concatenation: $[A; B]$ is the vertical, and $[A, B]$ the horizontal concatenation of two matrices with compatible dimensions.
We introduce the unitary Discrete Fourier Transform (DFT) operator $F_n$ on $\C^{n+1}$, defined by
\begin{align*}
\displaystyle
[F_{n} x]_k = \frac{1}{\sqrt{n+1}} \sum\limits_{t = 0}^n x_{t} \exp\left({\frac{2\pi i k t}{n+1}}\right), \quad 0 \le k \le n.
\end{align*}
The unitarity of $F_n$ implies that its inverse $F_n^{-1}$ coincides with its conjugate transpose $F_n^\H$.
Slightly abusing the notation, we will occasionally shorten $F_n [x]_0^n$ to $F_n[x]$. 
In other words, $F_n[\cdot]$ is a map $\C_n(\Z) \to \C^{n+1}$, and the adjoint map $F_n^\H[x]$ simply sends $F_n^\H [x]_0^n$ to $\C_n(\Z)$ via zero-padding.
%\[
%\|x\|_{n,p}^\F := \|F_n x\|_{n,p},
%\]

We use the ``Big-O'' notation: for two non-negative functions $g$, $f$ on the same domain, $g = \cO(f)$ means that there is a generic constant $C \ge 0$ such that $g \le Cf$ for any admissible value of the argument; $g = \tilde\cO(f)$ means that $C$ is replaced with $C(\log^{\kappa}(n)+1)$ for some $\kappa > 0$; hereinafter $\log(\cdot)$ is the natural logarithm, and $C$ a generic constant.

The signal denoising problem has attracted attention in statistical estimation and signal processing communities, see~\cite{ik1981,nemirovski_topics,tsybakov_mono,wasserman2006all,haykin1991adaptive,kay1993fundamentals} and references therein. 
The classical approach is to assume that the structure of the signal to recover, $x \in \C_n^{\pm}(\Z)$, is known to the statistician, and easy to exploit. 
This is usually attained by assuming that $x$ comes from a known subset $\X$ of $\C_n^{\pm}(\Z)$ with a simple structure.
For example, in parametric estimation, one considers linear subspaces $\S$ of $\C_n^\pm(\Z)$; in the nonparametric regression, one studies signals whose spectral-domain representation, as given by the Discrete Fourier or Discrete Wavelet transform, comes from a linearly transformed $\ell_p$-ball, see~\cite{tsybakov_mono,johnstone-book}. 
In all these cases, estimators with near-optimal statistical performance can be obtained in explicit form, and belong to the class of \textit{linear estimators} -- those linearly depending on the observations $y$. 

Unfortunately, such explicit characterization is usually unavailable when dealing with adaptive estimation problems. In these problems, the ``a priori'' set $\X$ is unspecified; instead, the signal is assumed to come from one of a large family $\{X_{\pi}\},$ $\pi \in \Pi$, of possible sets, which corresponds to one's uncertainty about the exact structure of the signal as specified by its support in the time or frequency domain, smoothness parameters, \textit{etc.}
The standard way to address such problems is by selecting an estimator in the family of near-minimax estimators for the sets $\X_\pi$ by minimizing a certain criterion of misfit.
%The search procedure is only allowed to use the available observations.
The hope is that the search procedure will manage to infer the necessary information from the available noisy observations,  resulting in the \textit{adaptive estimator} -- the one whose statistical performance is close to that of the unknown linear ``oracle'' estimator which ``knows'' the underlying structure. 
%-- near-minimax estimator for $X_{\pi^*}$ from which the signal ``truly'' comes.
%knows the actual set from which the signal ``truly'' comes. 
%Estimators with such property are called \textit{adaptive}.
Importantly, in order to be applicable in practice, an adaptive estimator must admit efficient algorithmic implementations. 
This puts additional limitations to the geometry of the family of possible linear estimators and the choice of misfit criterion.
%\dimacorr{}{Two fundamental examples of adaptive estimation problems are presented below.
%\begin{itemize}
%\item
%In \textit{sparse recovery}, $\{\X_\pi\}$ is the family of subspaces spanned by a small subset of elements of a fixed orthonormal basis.
% The known adaptive estimators in this case include the Lasso and the Dantzig selector~\cite{tibshirani,bickel2009simultaneous,candes2007dantzig}; both of them can be obtained as optimal solution of well-structured optimization problems, and, as such, are efficiently computable. 
%\item
%In \textit{smoothness adaptation}, each set $\X_\pi$ is an $\ell_p$-body which corresponds to a fixed choice of smoothness parameters for the function $f$ whose discretized version is $x$. As ``basic'' near-minimax estimators, one can often use kernel estimators, which correspond to the convolution of the observations with function $K_h(\cdot) = \frac{1}{h} K\left(\frac{\cdot}{h}\right)$, where $K: \R \to \R$ is a fixed \textit{kernel}  satisfying some regularity properties~\cite{tsybakov_mono}. The task is then to select the optimal bandwidth parameter $\wh h$ correspodning to the unknown smoothness information. This can be achieved, for example, via Lepski's method~\cite{lepski1991,lepski1997optimal,lepski2015adaptive}.
%\end{itemize}}
